SciExplore: Evaluating Autonomous Agents from Scientific Navigation to Information Integration

Scientific research involves complex information-seeking and reasoning workflows across heterogeneous sources. However, existing benchmarks primarily emphasize general-domain retrieval or static scientific question answering, and therefore fail to assess key capabilities required in realistic scientific research workflows. We introduce SciExplore, a benchmark designed to evaluate scientific information-seeking and reasoning capabilities of LLMs and agents. SciExplore comprises four task types covering 103 expert-curated tasks across more than ten scientific disciplines: scientific database navigation, ambiguous literature retrieval, missing reference completion, and cross-source structured knowledge synthesis, which probe progressively higher-level abilities from entity-level reasoning and document-level identification to evidence-level grounding and domain-level synthesis. We evaluate over ten state-of-the-art LLMs and autonomous agents on SciExplore, revealing substantial performance gaps with performance degrading sharply as task complexity increases and extremely low accuracy on the most challenging structured synthesis tasks. These results highlight significant limitations of current models and agents in realistic scientific information-seeking scenarios.

==> figs/overview.tex <==

\begin{figure}[!t]
            \centering
            \includegraphics[width=\linewidth]{figs/imgs/Overview.pdf}
            \vspace{-20pt}
            \caption{\textbf{Overview of our work.} (a) End-to-end LLMs directly convert papers into project pages, resulting in unreasonable layouts and lacking human feedback. (b) Our proposed AutoPage integrates human-agent collaboration into automated page generation with higher content and visual quality. The figure also illustrates the process for constructing the PageBench benchmark.} 
            
            % including data collection, test set construction, as well as the comprehensive evaluation metrics covering content quality and visual quality.
            
        
     \label{fig:overview}
    \vspace{-15pt}
\end{figure}

==> scripts/prompt_defs.tex <==
\definecolor{prompt}{RGB}{173, 216, 230}
\definecolor{prompt-frame}{RGB}{0, 51, 102}
\definecolor{prompt2}{RGB}{173, 216, 230}
\definecolor{prompt2-frame}{RGB}{0, 51, 102}
\definecolor{prompt3}{RGB}{173, 216, 230}
\definecolor{prompt3-frame}{RGB}{0, 51, 102}
\definecolor{prompt4}{RGB}{173, 216, 230}
\definecolor{prompt4-frame}{RGB}{0, 51, 102}
\definecolor{prompt5}{RGB}{173, 216, 230}
\definecolor{prompt5-frame}{RGB}{0, 51, 102}
\usepackage{fontawesome5}
\tcbset{
    prompt_func/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        overlay={
            \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        },
        title={~~~~~~~\textbf{Prompt used with GPT-4o to generate annotation for Element Grounding with functional setting}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}


\tcbset{
    full_content_generation/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Full Content Generation}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    filter_figures/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Filter Figures}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    section_generation/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Section Generation}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    html_generation/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: HTML Generation}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    full_content_review/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Full Content Review}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    full_content_revise/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Full Content Revise}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    text_content_generation/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Text Content Generation}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    html_review/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: HTML Review}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    html_revise/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: HTML Revise}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    prompt_aethetic_element/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Element Quality Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{
    prompt_aethetic_Layout/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Layout Balance Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_aethetic_engagement/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Engagement Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_info_clarity/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Clarity Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_info_content/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Content Completeness Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_info_logic/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Logical Flow Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}


\tcbset{prompt_verbatim_question/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Generate Verbatim QA}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_interpretive_question/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Generate Interpretive QA}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_answer_agent/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Answer Questions}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_4o_image/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: \texttt{4o-Image}}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_owl_4o/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: \texttt{OWL-4o}}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_4o_html/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: \texttt{4o-HTML}}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_parser_summarizer/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Paper Summarizer}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_parser_filter/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Figure Filter}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}


\tcbset{prompt_planner_matching/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Asset Matching}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_planner_painter/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Painter}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{prompt_planner_commenter/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {\faDatabase};
        % },
        title={\faDatabase~~~\textbf{Prompt: Commenter}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}


\tcbset{
    vlm_aesthetics_judge/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Aesthetics Quality Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}
\tcbset{
    vlm_element_judge/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Element Quality Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

\tcbset{
    vlm_layout_judge/.style={
        enhanced,
        breakable,
        colback=prompt,        % Background color
        colframe=prompt-frame,            % Frame color
        fontupper=\normalsize,               % Monospace font
        boxrule=1pt,                       % Frame thickness
        arc=4mm,                           % Rounded corners
        left=1mm, right=1mm, top=1mm, bottom=1mm, % Padding
        boxsep=4pt,                        % Space between text and box
        before skip=10pt, after skip=10pt, % Vertical spacing
        % overlay={
        %     \node[anchor=north west, xshift=4pt, text=white] at (frame.north west) {};
        % },
        title={\faDatabase~~~\textbf{Prompt: Layout Quality Judge}},
        coltitle=white,
        fonttitle=\bfseries\small
    }
}

==> tabs/ablation.tex <==
% \begin{table*}[ht!]
% \centering
% \caption{Ablation study on different verifiers.}
% \label{tab:ablation_verfier}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Ablate Component}} & \multicolumn{3}{c|}{\textbf{Content Quality}} & \multicolumn{3}{c}{\textbf{Visual Quality}} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% & \begin{tabular}[c]{@{}c@{}}Readability \end{tabular} & \begin{tabular}[c]{@{}c@{}}Semantic Fidelity \end{tabular} & \begin{tabular}[c]{@{}c@{}}Compression-Aware \\ Information Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Visual Content  \\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Layout and \\ Cohesion\end{tabular} & Aesthetic Score \\
% \midrule
% \quad AutoPage &11.090 &0.739 &1.744 &3.13 &2.15 &2.69 \\
% \midrule
% \quad \texttt{w/o} Full Content Checker &10.745 &0.695 &1.533 &3.05 &1.95 &2.25 \\
% \quad \texttt{w/o} HTML Checker &10.795 &0.708 &1.583 &2.90 &1.65 &2.20 \\
% \quad \texttt{w/o} all checkers &10.745 &0.695 &1.533 &2.75 &1.60 &1.90 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% The best performance for each metric is in \textbf{bold}, and the second best is \underline{underlined}.

\begin{table}[h!] % 在单栏环境下，可以用 [ht!] 替代 [ht!]
\centering
\caption{\textbf{Ablation study on different verifiers of AutoPage.}}
\vspace{-10pt}
\label{tab:ablation_verfier}
\resizebox{\linewidth}{!}{
\begin{tabular}{l cccc}
\toprule
& & \multicolumn{3}{c}{\textbf{\texttt{w/o} Verifier}} \\
\cmidrule(lr){3-5}
\textbf{Metric} & {\textbf{AutoPage}} & {Full Content} & {HTML} & {All} \\
\midrule
\multicolumn{5}{l}{\textit{Content Quality}} \\
\quad Readability$\downarrow$ & \textbf{10.090} & \underline{10.745} & 10.795 & \underline{10.745} \\
\quad Semantic Fidelity$\uparrow$  & \textbf{0.739} & 0.695 & \underline{}{0.708} & 0.695 \\
\quad Comp.-Aware Info. Acc. $\uparrow$ & \textbf{1.744} & 1.533 & \underline{1.583} & 1.533 \\
\midrule
\multicolumn{5}{l}{\textit{Visual Quality}} \\
\quad Visual Content Acc. $\uparrow$ & \textbf{3.13} & \underline{}{3.05} & 2.90 & 2.75 \\
\quad Layout and Cohesion $\uparrow$ & \textbf{2.15} & \underline{1.95} & 1.65 & 1.60 \\
\quad Aesthetic Score $\uparrow$ & \textbf{2.69} & \underline{2.25} & 2.20 & 1.90 \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table}


% \begin{table}[ht!]
% \centering
% \caption{Ablation study on different verifiers.}
% \label{tab:ablation_verfier}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Ablate Component}} & \multicolumn{3}{c}{\textbf{Content Quality}} \\
% \cmidrule(lr){2-4}
% & \begin{tabular}[c]{@{}c@{}}Readability \end{tabular} & \begin{tabular}[c]{@{}c@{}}Semantic Fidelity \end{tabular} & \begin{tabular}[c]{@{}c@{}}Compression-Aware \\ Information Accuracy\end{tabular} \\
% \midrule
% \quad AutoPage &11.090 &0.739 &1.744 \\
% \midrule
% \quad \texttt{w/o} Full Content Checker & & & \\
% \quad \texttt{w/o} HTML Checker &10.795 &0.708 &1.583 \\
% \quad \texttt{w/o} all checkers &10.745 &0.695 &1.533 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{table}[ht!]
% \centering
% \caption{Ablation study on different verifiers.}
% \label{tab:ablation_verfier}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Ablate Component}} & \multicolumn{3}{c}{\textbf{Visual Quality}} \\
% \cmidrule(lr){2-4}
% & \begin{tabular}[c]{@{}c@{}}Visual Content  \\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Layout and \\ Cohesion\end{tabular} & Aesthetic Score \\
% \midrule
% \quad AutoPage &3.13 &2.15 &2.69 \\
% \midrule
% \quad \texttt{w/o} Full Content Checker &3.05 &1.95 &2.25 \\
% \quad \texttt{w/o} HTML Checker &2.90 &1.65 &2.20 \\
% \quad \texttt{w/o} all checkers &2.75 &1.60 &1.90 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


==> tabs/main_exp.tex <==
% \begin{table*}[hbtp]
% \centering
% \caption{Main Results}
% \label{tab:main_results}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Content Quality}} & \multicolumn{3}{c}{\textbf{Visual Quality}} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% & \begin{tabular}[c]{@{}c@{}}Readability \end{tabular} & \begin{tabular}[c]{@{}c@{}}Semantic Fidelity \end{tabular} & \begin{tabular}[c]{@{}c@{}}Compression-Aware \\ Information Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Visual Content  \\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Layout and \\ Cohesion\end{tabular} & Aesthetic Score \\
% \midrule
% \multicolumn{7}{l}{\textbf{End2End (open-source)}} \\
% \quad Qwen3-235B-A22B &11.590 &0.571 &1.890 &2.52 &1.93 &2.46 \\
% \quad GPT-OSS-120B &9.665 &0.608 &1.719 &2.74 &1.82 &2.65 \\
% \quad llama-3.1-70B &15.967 &0.442 &1.270 &2.52 &1.78 &2.41 \\

% \midrule
% \multicolumn{7}{l}{\textbf{End2End (close-source)}} \\
% \quad Grok4-fast &14.101 &0.603 &1.808 &2.68 &2.01 &2.67 \\
% \quad GLM-4.5-Air &10.568 &0.587 &1.788 &2.98 &2.03 &2.67 \\
% \quad GPT4o-mini &10.047 &0.554 &1.786 &2.96 &2.08 &2.71 \\
% \quad Gemini2.5-Flash &11.343 &0.684 &1.276 &2.82 &2.00 &2.48 \\
% \midrule
% \multicolumn{7}{l}{\textbf{AutoPage-Variants}} \\
% \quad AutoPage-GPT4o-mini &10.819 &0.621 &1.837 &3.08 &2.38 &2.95 \\
% \quad AutoPageGemini-2.5-Flash &10.992 &0.742 &1.941 &3.13 &2.15 &2.69 \\
% \quad AutoPage-Qwen &10.425 &0.663 &1.591 &3.01 &2.28 &2.72 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[hbtp]
\centering
\caption{\textbf{Main evaluation results across our full suite of PageBench.} The best performance among all methods for each metric is in \textbf{bold}, and the second best is \underline{underlined}. For ease of comparison, AutoPage and its corresponding proprietary base models are highlighted in matching colors. AutoPage improves both content and visual quality over different base models, validating its effectiveness in producing accurate, coherent, and visually refined webpages. }
\vspace{-10pt}
\label{tab:main_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{System Type}} & \multirow{2}{*}{\textbf{Open-Source}} & \multicolumn{3}{c|}{\textbf{Content Quality}} & \multicolumn{3}{c}{\textbf{Visual Quality}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
 &  &  & \begin{tabular}[c]{@{}c@{}}Readability \textbf{$\downarrow$}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semantic\\ Fidelity \textbf{$\uparrow$}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Comp.-Aware \\ Info. Acc. \textbf{$\uparrow$} \end{tabular} & \begin{tabular}[c]{@{}c@{}}Visual Content\\ Accuracy \textbf{$\uparrow$} \end{tabular} & \begin{tabular}[c]{@{}c@{}}Layout and\\ Cohesion\textbf{$\uparrow$}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Aesthetic\\ Score\textbf{$\uparrow$}\end{tabular} \\
\midrule
% \quad Qwen3-235B-A22B &E2E  &\textcolor{gray}{\usym{2714}} & 11.590 & 0.571 & \underline{1.890} & 2.52 & 1.93 & 2.46 \\
\quad GPT-OSS-120B & E2E &\textcolor{gray}{\usym{2714}} & \textbf{9.665} & 0.608 & 1.719 & 2.74 & 1.82 & 2.65 \\
\quad llama-3.1-70B &E2E  &\textcolor{gray}{\usym{2714}} & 15.967 & 0.442 & 1.270 & 2.52 & 1.78 &2.41 \\

% \midrule
\quad Grok4-fast &E2E  & & 14.101 & 0.603 & 1.808 & 2.68 & 2.01 & 2.67 \\
\quad GLM-4.5-Air & E2E & & 10.568 & 0.587 & 1.788 & 2.98 & 2.03 & 2.67 \\
% \rowcolor{lightcoral}\quad GPT4o-mini &  & & \underline{10.047} & 0.554 & 1.786 & 2.96 & 2.08 & 2.71 \\
% \rowcolor{skyblue}\quad Gemini2.5-Flash &  & & 11.343 & \underline{0.684} & 1.276 & 2.82 & 2.00 & 2.48 \\

\midrule
\quad Qwen3-235B-A22B &E2E  &\textcolor{gray}{\usym{2714}} & 11.590 & 0.571 & \underline{1.890} & 2.52 & 1.93 & 2.46 \\
\rowcolor{lemonchiffon}\quad AutoPage-Qwen &Multi-Agent & & 10.425 & 0.663 & 1.837 & 3.01 & 2.28 & 2.72 \\
\midrule
\quad GPT4o-mini &E2E  & & \underline{10.047} & 0.554 & 1.786 & 2.96 & 2.08 & 2.71 \\
\rowcolor{lightcoral}\quad AutoPage-GPT4o-mini &Multi-Agent  & & 10.819 & 0.621 & \textbf{1.941} & 3.08 & \underline{2.38} & \underline{2.95} \\
\midrule
\quad Gemini2.5-Flash &E2E  & & 11.343 &0.684 & 1.276 & 2.82 & 2.00 & 2.48 \\
\rowcolor{skyblue}\quad AutoPage-Gemini2.5-Flash & Multi-Agent & & 10.992 & 
\textbf{0.742} & 1.591 & \textbf{3.13} & 2.15 & 2.69 \\
\midrule
\quad GPT5-mini & E2E & &  11.964 & 0.6308 & 1.589 & 2.99 &2.12 & 2.74 \\
\rowcolor{SeaGreen} \quad AutoPage-GPT5-mini &Multi-Agent & &10.709 & \underline{0.7015} & 1.818 & \underline{3.11} &\textbf{2.40} & \textbf{2.96} \\

\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table*}


% \begin{table*}[t!]
% \centering
% \caption{Main evaluation results across our full suite of \textbf{PageBench} (transposed format). 
% The best performance for each metric is in \textbf{bold}, and the second best is \underline{underlined}.
% AutoPage models and their corresponding proprietary base models share matching highlight colors.}
% \label{tab:main_results_transposed_grouped}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccc|cccc|ccc}
% \toprule
% & \multicolumn{3}{c|}{\textbf{E2E (Open-source)}} & \multicolumn{4}{c|}{\textbf{E2E (Close-source)}} & \multicolumn{3}{c}{\textbf{Multi-Agent System}} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-11}
% \textbf{Metric} & Qwen3-235B-A22B & GPT-OSS-120B & llama-3.1-70B &
% Grok4-fast & GLM-4.5-Air & \cellcolor{lightcoral}GPT4o-mini & \cellcolor{skyblue}Gemini2.5-Flash &
% \cellcolor{lightcoral}AutoPage-GPT4o-mini & \cellcolor{skyblue}AutoPage-Gemini2.5-Flash & AutoPage-Qwen \\
% \midrule
% \multicolumn{11}{l}{\textit{Content Quality}} \\
% \quad Readability $\downarrow$ & 11.590 & \textbf{9.665} & 15.967 & 14.101 & 10.568 & \underline{10.047} & 11.343 & 10.819 & 10.992 & 10.425 \\
% \quad Semantic Fidelity $\uparrow$ & 0.571 & 0.608 & 0.442 & 0.603 & 0.587 & 0.554 & \underline{0.684} & 0.621 & \textbf{0.742} & 0.663 \\
% \quad Comp.-Aware Info. Acc. $\uparrow$ & \underline{1.890} & 1.719 & 1.270 & 1.808 & 1.788 & 1.786 & 1.276 & 1.837 & \textbf{1.941} & 1.591 \\
% \midrule
% \multicolumn{11}{l}{\textit{Visual Quality}} \\
% \quad Visual Content Accuracy $\uparrow$ & 2.52 & 2.74 & 2.52 & 2.68 & 2.98 & 2.96 & 2.82 & \underline{3.08} & \textbf{3.13} & 3.01 \\
% \quad Layout \& Cohesion $\uparrow$ & 1.93 & 1.82 & 1.78 & 2.01 & 2.03 & 2.08 & 2.00 & \textbf{2.38} & \underline{2.15} & 2.28 \\
% \quad Aesthetic Score $\uparrow$ & 2.46 & 2.65 & 2.41 & 2.67 & 2.67 & 2.71 & 2.48 & \textbf{2.95} & \underline{2.69} & 2.72 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}







==> tabs/pageagent-variants.tex <==
\begin{table*}[ht!]
\centering
\caption{AutoPage with different LLM backbone.}
\label{tab:variants}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{LLM-Backbone}} & \multicolumn{3}{c|}{\textbf{Content Quality}} & \multicolumn{3}{c}{\textbf{Visual Quality}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \begin{tabular}[c]{@{}c@{}}Readability \end{tabular} & \begin{tabular}[c]{@{}c@{}}Semantic Fidelity \end{tabular} & \begin{tabular}[c]{@{}c@{}}Compression-Aware \\ Information Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Visual Content  \\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Layout and \\ Cohesion\end{tabular} & Aesthetic Score \\
\midrule
\quad AutoPage-GPT4o & & & & & & \\
\quad AutoPage-Gemini & & & & & & \\
\quad AutoPage-Qwen & & & & & & \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tabs/qa.tex <==
\begin{table*}[hbtp]
\centering
\caption{\textbf{Performance Comparison across Different Methods.} The best performance among all methods for each metric is in \textbf{bold}, and the second best is \underline{underlined}. For ease of comparison, AutoPage and its corresponding proprietary base models are highlighted in matching colors. The compression rate is also listed in the table. }
\vspace{-10pt}
\label{tab:qa_performance}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcc|ccc|ccc|c|c|ccc}
\toprule
\multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{System Type}} & \multirow{3}{*}{\textbf{Open-Source}} & \multicolumn{7}{c|}{\textbf{Raw-ACC}} & \multirow{3}{*}{\textbf{Compression}} & \multicolumn{3}{c}{\textbf{Compression-Aware ACC}} \\
\cmidrule(lr){4-10} \cmidrule(lr){12-14}
 &  &  & \multicolumn{3}{c|}{\textbf{Detail question}} & \multicolumn{3}{c|}{\textbf{Understanding question}} & \multirow{2}{*}{\textbf{Overall}$\uparrow$} &  & \multirow{2}{*}{\textbf{D-Avg}$\uparrow$} & \multirow{2}{*}{\textbf{U-Avg}$\uparrow$} & \multirow{2}{*}{\textbf{Overall$\uparrow$}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
 &  &  & \begin{tabular}[c]{@{}c@{}}Open-\\Source\end{tabular} & \begin{tabular}[c]{@{}c@{}}Close-\\Source\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{D-Avg}$\uparrow$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Open-\\Source\end{tabular} & \begin{tabular}[c]{@{}c@{}}Close-\\Source\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{U-Avg}$\uparrow$\end{tabular} &  &  &  &  \\
\midrule
\quad GPT-OSS-120B & E2E & \textcolor{gray}{\usym{2714}} & 0.662 & 0.617 & 0.640 & 0.869 & 0.844 & 0.856 & 0.748 & 10.833 & 1.469 & 1.970 & 1.719 \\
\quad llama-3.1-70B & E2E & \textcolor{gray}{\usym{2714}} & 0.422 & 0.218 & 0.320 & 0.617 & 0.380 & 0.499 & 0.409 & 29.594 & 0.992 & 1.548 & 1.270 \\
\quad Grok-4-fast & E2E &  & \underline{0.725} & \underline{0.711} & \underline{0.718} & 0.880 & \underline{0.890} & \textbf{0.885} & \underline{0.801} & 10.347 & \underline{1.617} & 1.999 & 1.808 \\
\quad GLM-4.5-Air & E2E &  & 0.688 & 0.619 & 0.653 & \underline{0.905} & 0.850 & \underline{0.877} & 0.765 & 11.213 & 1.526 & 2.049 & 1.788 \\
\midrule
\quad Qwen3-235B-A22B & E2E & \textcolor{gray}{\usym{2714}} & 0.692 & 0.547 & 0.620 & 0.859 & 0.794 & 0.826 & 0.723 & 15.931 & \textbf{1.659} & \underline{2.121} & \underline{1.890} \\
\rowcolor{lemonchiffon}\quad AutoPage-Qwen & Multi-Agent &  & 0.700 & 0.635 & 0.668 & \textbf{0.914} & 0.833 & 0.874 & 0.771 & 11.592 & 1.593 & 2.081 & 1.837 \\
\midrule
\quad GPT-4o-mini & E2E &  & 0.635 & 0.374 & 0.505 & 0.838 & 0.606 & 0.722 & 0.613 & 20.045 & 1.472 & 2.099 & 1.786 \\
\rowcolor{lightcoral}\quad AutoPage-GPT-4o-mini & Multi-Agent &  & 0.635 & 0.398 & 0.517 & 0.899 & 0.662 & 0.781 & 0.649 & 23.528 & 1.581 & \textbf{2.389} & \textbf{1.941} \\
\midrule
\quad Gemini-2.5-flash & E2E &  & \textbf{0.735} & \textbf{0.723} & \textbf{0.729} & 0.869 & \textbf{0.901} & \textbf{0.885} & \textbf{0.807} & 5.302 & 1.150 & 1.402 & 1.276 \\
\rowcolor{skyblue}\quad AutoPage-Gemini-2.5-flash & Multi-Agent &  & 0.715 & 0.687 & 0.701 & 0.882 & 0.870 & 0.876 & 0.788 & 8.419 & 1.411 & 1.770 & 1.591 \\
\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table*}

% \begin{table*}[hbtp]
% \centering
% \caption{\textbf{Performance Comparison across Different Methods.} The best performance among all methods for each metric is in \textbf{bold}, and the second best is \underline{underlined}. }
% \vspace{-10pt}
% \label{tab:performance}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcc|ccc|ccc|c|c|ccc}
% \toprule
% \multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{System Type}} & \multirow{3}{*}{\textbf{Open-Source}} & \multicolumn{7}{c|}{\textbf{Raw-ACC}} & \multirow{3}{*}{\textbf{Compression}} & \multicolumn{3}{c}{\textbf{Compression-Aware ACC}} \\
% \cmidrule(lr){4-10} \cmidrule(lr){12-14}
%  &  &  & \multicolumn{3}{c|}{\textbf{Detail question}} & \multicolumn{3}{c|}{\textbf{Understanding question}} & \multirow{2}{*}{\textbf{Overall}$\uparrow$} &  & \multirow{2}{*}{\textbf{D-Avg}$\uparrow$} & \multirow{2}{*}{\textbf{U-Avg}$\uparrow$} & \multirow{2}{*}{\textbf{Overall}$\uparrow$} \\
% \cmidrule(lr){4-6} \cmidrule(lr){7-9}
%  &  &  & \begin{tabular}[c]{@{}c@{}}Open-\\Source\end{tabular} & \begin{tabular}[c]{@{}c@{}}Close-\\Source\end{tabular} & \textbf{D-Avg}$\uparrow$ & \begin{tabular}[c]{@{}c@{}}Open-\\Source\end{tabular} & \begin{tabular}[c]{@{}c@{}}Close-\\Source\end{tabular} & \textbf{U-Avg}$\uparrow$ &  &  &  &  & \\
% \midrule
% \quad GPT-OSS-120B & E2E & \textcolor{gray}{\usym{2714}} & 0.662 & 0.617 & 0.640 & 0.869 & 0.844 & 0.856 & 0.748 & 10.833 & 1.469 & 1.970 & 1.719 \\
% \quad llama-3.1-70B & E2E & \textcolor{gray}{\usym{2714}} & 0.422 & 0.218 & 0.320 & 0.617 & 0.380 & 0.499 & 0.409 & 29.594 & 0.992 & 1.548 & 1.270 \\
% \quad Grok-4-fast & E2E &  & \underline{0.725} & \underline{0.711} & \underline{0.718} & 0.880 & \underline{0.890} & \textbf{0.885} & \underline{0.801} & 10.347 & \underline{1.617} & 1.999 & 1.808 \\
% \quad GLM-4.5-Air & E2E &  & 0.688 & 0.619 & 0.653 & \underline{0.905} & 0.850 & \underline{0.877} & 0.765 & 11.213 & 1.526 & 2.049 & 1.788 \\
% \midrule
% \quad Qwen3-235B-A22B & E2E & \textcolor{gray}{\usym{2714}} & 0.692 & 0.547 & 0.620 & 0.859 & 0.794 & 0.826 & 0.723 & 15.931 & \textbf{1.659} & \underline{2.121} & \underline{1.890} \\
% \rowcolor{lemonchiffon}\quad AutoPage-Qwen & Multi-Agent &  & 0.700 & 0.635 & 0.668 & \textbf{0.914} & 0.833 & 0.874 & 0.771 & 11.592 & 1.593 & 2.081 & 1.837 \\
% \midrule
% \quad GPT-4o-mini & E2E &  & 0.635 & 0.374 & 0.505 & 0.838 & 0.606 & 0.722 & 0.613 & 20.045 & 1.472 & 2.099 & 1.786 \\
% \rowcolor{lightcoral}\quad AutoPage-GPT-4o-mini & Multi-Agent &  & 0.635 & 0.398 & 0.517 & 0.899 & 0.662 & 0.781 & 0.649 & 23.528 & 1.581 & \textbf{2.389} & \textbf{1.941} \\
% \midrule
% \quad Gemini-2.5-flash & E2E &  & \textbf{0.735} & \textbf{0.723} & \textbf{0.729} & 0.869 & \textbf{0.901} & \textbf{0.885} & \textbf{0.807} & 5.302 & 1.150 & 1.402 & 1.276 \\
% \rowcolor{skyblue}\quad AutoPage-Gemini-2.5-flash & Multi-Agent &  & 0.715 & 0.687 & 0.701 & 0.882 & 0.870 & 0.876 & 0.788 & 8.419 & 1.411 & 1.770 & 1.591 \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-15pt}
% \end{table*}

